Fully Aligned Network for Referring Image Segmentation

This paper focuses on the Referring Image Segmentation (RIS) task, which aims to segment objects from an image based on a given language description. The critical problem of RIS is achieving fine-grained alignment between different modalities to recognize and segment the target object. Recent advances using the attention mechanism for cross-modal interaction have achieved excellent progress. However, current methods tend to lack explicit principles of interaction design as guidelines, leading to inadequate cross-modal comprehension. Additionally, most previous works use a single-modal mask decoder for prediction, losing the advantage of full cross-modal alignment. To address these challenges, we present a Fully Aligned Network (FAN) that follows four cross-modal interaction principles. Under the guidance of reasonable rules, our FAN achieves state-of-the-art performance on the prevalent RIS benchmarks (RefCOCO, RefCOCO+, G-Ref) with a simple architecture.

==> Tables/text_encoder.tex <==
\begin{table}[t]
    \centering
    \caption{Experiments results of different text encoder on RefCOCO validation set.}
    \vspace{-5pt}
    \small
    \label{tab:text_encoder}
    \setlength\tabcolsep{4pt}
    \begin{tabular}{lcccccc}
        \toprule[1pt]
        Encoder &IoU & P@0.5 & P@0.6 & P@0.7 & P@0.8 & P@0.9 \\
        \midrule
        Bert~\cite{bert}  &73.76 &85.16 &81.06 &75.24 &61.49 &24.08\\
        CLIP~\cite{CLIP}	&74.06 &85.82 &82.04 &75.69 &61.77 &24.77\\
        \bottomrule[1pt]
    \vspace{-20pt}
    \end{tabular}
    \end{table}

==> Tables/text_encoder_setting.tex <==
\begin{table}[t]
    \caption{Experiments on different text encoder and whether to freeze them during training. The visual backbone in these experiments is Swin-B.}
   \centering
   \footnotesize
%   \renewcommand\arraystretch{1.1}
   \resizebox{\columnwidth}{!}{\begin{tabular}{l|c|c|c|c}
      \toprule[1pt]
      % \hline
      & IoU & P@0.5 & P@0.7 & P@0.9\\
      % \bottomrule[1pt]
      \hline
      \multicolumn{5}{l}{ \textbf{(a)} Different Text Encoder} \\
      % \toprule[1pt]
      \hline
      CLIP Text Encoder & 74.06 & 85.82 & 75.69 & 24.77  \\
      Bert & 73.66 & 85.24 & 75.36 & 24.08\\
      % \bottomrule[1pt]
      \hline
      \multicolumn{5}{l}{ \textbf{(b)} Training Settings} \\
      % \toprule[1pt]
      \hline
      Freeze Bert  & 71.09 & 81.67 & 70.86 & 22.03 \\
    %   Finetune  & \textbf{84.46} & \textbf{75.28} & \textbf{34.30} & \textbf{72.73}  \\
      Finetune Bert  & 73.66 & 85.16 & 75.24 & 24.08 \\
      Freeze CLIP Text Encoder & 73.96???? & 85.32 & 75.75 & 24.28 \\
      Finetue CLIP Text Encoder & 74.06 & 85.82 & 75.69 & 24.77 \\
      \bottomrule[1pt]
      % \hline
   \end{tabular}}
   
   \label{tab:text_encoder}
\end{table}
